Nonlinear MPC for Quadrotor Fault-Tolerant Control

The mechanical simplicity, hover capabilities, and high agility of quadrotors lead to a fast adaption in the industry for inspection, exploration, and urban aerial mobility. On the other hand, the unstable and underactuated dynamics of quadrotors render them highly susceptible to system faults, especially rotor failures. In this work, we propose a fault-tolerant controller using nonlinear model predictive control (NMPC) to stabilize and control a quadrotor subjected to the complete failure of a single rotor. Differently from existing works, which either rely on linear assumptions or resort to cascaded structures neglecting input constraints in the outer-loop, our method leverages full nonlinear dynamics of the damaged quadrotor and considers the thrust constraint of each rotor. Hence, this method could effectively perform upset recovery from extreme initial conditions. Extensive simulations and real-world experiments are conducted for validation, which demonstrates that the proposed NMPC method can effectively recover the damaged quadrotor even if the failure occurs during aggressive maneuvers, such as flipping and tracking agile trajectories.

==> sections/related_work.tex <==
\subsection{Related Work}\label{sec:related_work}
FTFC is a long-standing challenge within the robotics and aerospace industries.
Initial research focused on partial effectiveness loss of rotors, such as blade damage, where a quadrotor is mainly regarded as a research platform for testing novel robust/adaptive control methods.
These methods include but are not limited to sliding mode control~\cite{wang2019quadrotor,Besnard2012}, $\mathcal{L}_1$ adaptive control~\cite{Xu2016}, and active disturbance rejection control~\cite{Guo2018}.
Extensive research on fault detection and diagnosis is also carried out and tested on quadrotor platforms (e.g., see~\cite{amoozgar2013experimental,freddi2010actuator}).

While partial motor failure can be effectively handled by these adaptive methods, failure of a complete rotor is a more challenging problem and has a higher practical value.
This is because switching off a severely damaged rotor in practice is more favorable as it prevents vibrations caused by rotor imbalance.
A seminal work to address this problem is proposed by~\cite{freddi_feedback_2011} which reveals that relinquishing the stability in yaw direction is inevitable after the failure of a motor.
But even then, the altitude and position of a post-failure quadrotor remain controllable.
Based on this seminal work \cite{freddi_feedback_2011} a wide variety of methods have been proposed and tested, including linear controllers such as proportional-integral-derivative (PID) controlller~\cite{lippiello_emergency_2014-1}, linear quadratic regulator (LQR)~\cite{mueller_stability_2014}, and linear parameter varying (LPV)~\cite{stephan_linear_2018} methods that rely on a relaxed hovering equilibrium to perform linearization~\cite{mueller2016relaxed}. 
Nonlinear methods that are independent of this hovering solution have also been proposed, including robust feedback linearization~\cite{lanzon_flight_2014}, nonlinear dynamic inversion (NDI)~\cite{sun2021autonomous}, backstepping~\cite{lippiello_emergency_2014}, and incremental nonlinear dynamic inversion (INDI)~\cite{sun_incremental_2020,sun_high-speed_2018}.
Recently, vision-based approaches~\cite{sun2021autonomous} jointly addressed the control and state estimation problem using only onboard sensors.

These methods, however, rely on different assumptions for controller design, such as small-angle assumptions for model linearization or the principle of time-scale separations for separately designing position and attitude controllers.
Moreover, they do not consider actuator limits, which are crucial for flight performance, especially after rotor failures.
For this reason, the nonlinear model predictive controller, that exploits the full dynamics of a quadrotor, is a perfect candidate to tackle the fault-tolerant control problem. 
% The first flight controller resilience to complete failure of a single rotor was proposed by \cite{freddi_feedback_2011} using a feedback linearization approach. The authors demonstrated that relinquishing the stability in the yaw direction becomes inevitable in order to keep the full control of pitch, roll, and thrust. As a consequence, the drone fast spins due to the imbalanced drag torques from remaining rotors. Following this idea, different approaches were proposed for this problem, such as PID~\cite{lippiello_emergency_2014-1}, backstepping~\cite{lippiello_emergency_2014}, robust feedback linearization \cite{lanzon_flight_2014}, and INDI \cite{lu_active_2015}. However, these works were only validated in simulation environments.

% The first real-world flight test of a quadrotor with a complete failure of a rotor was achieved by~\cite{mueller_stability_2014}, where a linear quadratic regulator (LQR) was applied. The authors also proposed the \textit{relaxed-hovering solution} as a quasi-equilibrium, where the quadrotor spins about a fixed point in the 3-D space, with constant body rates, pitch, and roll angles~\cite{mueller_relaxed_2016}. The authors proposed to use open-loop control to first accumulate body yaw rate near a relaxed-hovering solution and then engage the LQR, which is based on a linearized model around the the solution.
% The authors of \cite{stephan_linear_2018} used a linear parameter varying controller, in which a linearized model dependent on the body yaw rate was used for control.
% The INDI approach was applied in \cite{sun_high-speed_2018} and \cite{sun_incremental_2020}, where the authors considered fault-tolerant control in high-speed flights. INDI renders the controller resilient to significant aerodynamic disturbances in high-speed wind-tunnel flight tests.

NMPC is a control method that uses a nonlinear model to predict the system dynamics from a current time over a receding horizon and optimizes the behavior of the system based on certain performance measurements.
It was shown in previous research that NMPC on quadrotors has a great advantage in agile trajectory tracking and dealing with constraints \cite{Foehn_2021, bangura_real-time_2014, kamel_fast_2015}. 
Due to the ability of the NMPC to fully exploit the input space without constraint violation, it was tested as the FTFC to stabilize a hexacopter with a rotor failure in~\cite{kamel_fast_2015}, although the loss of a single rotor is not a challenging situation for hexacopter control.
A more difficult case was tested, in which three rotors fail on a hexacopter~\cite{aoki_nonlinear_2018}.
It was shown with simulations that the nonlinear NMPC controls the horizontal position and maintains the altitude of the drone.
The authors of \cite{jung_fault_2021} also proposed a method using MPC as the inner loop controller for a quadrotor subject to rotor failures, which is only validated in the simulation in near-hovering flights. 

However, NMPC has several disadvantages that make it difficult to be implemented in the real world \cite{darby_mpc_2012} \cite{eren_model_2017}.
To obtain good predictions it is necessary to accurately model the system dynamics, which is particularly challenging for aerial robots whose dynamics are severely influenced by aerodynamic effects.
The complexity of the optimization problem also makes NMPC difficult to satisfy the requirements for real-time control.
As a result, NMPC has never been implemented in real-world experiments to control a quadrotor in the case of a complete failure of a rotor.
Thus in this work, we implement the nonlinear NMPC onboard a quadrotor platform to perform real-world flights.
A combination of NMPC with INDI, as is proposed in a previous work~\cite{sun2021comparative}, is also adopted to compensate for the model uncertainties.
